Exploring the Opportunities of AR for Enriching Storytelling with Family Photos between Grandparents and Grandchildren

Storytelling with family photos, as an important mode of reminiscence-based activities, can be instrumental in promoting intergenerational communication between grandparents and grandchildren by strengthening generation bonds and shared family values. Motivated by challenges that existing technology approaches encountered for improving intergenerational storytelling (e.g., the need to hold the tablet, the potential view detachment from the physical world in Virtual Reality (VR)), we sought to find new ways of using Augmented Reality (AR) to support intergenerational storytelling, which offers new capabilities (e.g., 3D models, new interactivity) to enhance the expression for the storyteller. We conducted a two-part exploratory study, where pairs of grandparents and grandchildren 1) participated in an in-person storytelling activity with a semi-structured interview 2) and then a participatory design session with AR technology probes that we designed to inspire their exploration. Our findings revealed insights into the possible ways of intergenerational storytelling, the feasibility and usages of AR in facilitating it, and the key design implications for leveraging AR in intergenerational storytelling.

==> rebuttal.tex <==
1. Why AR?  

comparison with tablet-based ST


AR usage: Most of the used functionality and finding does not strongly link to AR. Most could be achieved by using a tablet and it is not clear how users benefit from AR (with very few exceptions). This link needs to be clearer throughout large parts of the paper (Intro, Probe Design, Findings). On the other hand, the authors found throughout their analysis challenges that arose because of the usage of AR. I was wondering if AR war a good idea or perhaps not.

% 沉浸感、可视化、强交互的功能只有AR能提供

Setup: It is unclear why the authors chose to use a single AR device when investigating collocated storytelling. Wouldn’t the experience benefit from a symmetric setup?

% 我们研究中，讲故事的主体是老人，AR主要是用于帮助老人更好地讲故事，年轻人可以通过屏幕获得实时的反馈。我们


Findings: Some of the findings are in general interesting but also feel sometimes quite obvious (e.g., AR could use other modalities) or not AR related (e.g., AI could be used). While it could be okay in general, it somehow feels odd given the framing of the paper.

% 我们有general的findings，也有AR-specific的findings，所有的finding都是为AR在storytelling中的adaptivity和feasibility服务的。我们会在revision中进一步优化。

Probes: I appreciate the usage of probes. However, they do not really showcase the benefit of AR. Pointing at someone, playing background music, or restoring a photo is not linked to AR at all. The display and manipulation of 3 models might be attributed to AR although it can also be done on a mobile/desktop setup. Some more rationale for the selection of these probes could help to make them stronger.

% 用户是新手，不适合太复杂的功能，我们给的是一些引导性的probe，帮助用户熟悉沉浸式环境和3D对象交互。pointing和music是AR中基础的交互、反馈模式，XXXX。我们会在revision中进一步优化。

A: Thanks for your valuable comments. 
Given our participants were all novice to AR xxx. 

immersive environment XXX, 

As Our probe study has two main goals: 

We will make further clarification on this point in our revision. 
